Top quark spin and quantum entanglement in the ATLAS experiment

Top quark pair spin correlation measurements performed by the ATLAS experiment using $pp$ collisions at the CERN Large Hadron Collider are summarized. Moreover, the measurement of a specific observable $D$ related to top quark pair spin correlations is presented using the full LHC Run 2 data taking at the center-of-mass energy of $\sqrt{s} = 13$ TeV. This allowed the ATLAS experiment to observe the quantum entanglement, one of the fundamental property of the quantum mechanics.

==> Makefile <==
###############################################################################
#                                                       
#
# Makefile for a TOP2024 proceedings
#
###############################################################################

#main settings
PDFLATEX = pdflatex
LATEX    = latex
BIBTEX   = bibtex
#BIBTEX   = biber
DVIPDF   = dvipdf
DVIPS    = dvips

# The main document filename
BASENAME = SciPost_Proceedings_TOP2024_Lysak

#graphics_eps := $(wildcard *.eps)
#graphics_pdf := $(patsubst %.eps,%.pdf,$(wildcard *.eps))
graphics_pdf := $(wildcard *fig*.pdf)
tex_files := $(wildcard *.tex)
aux_files := $(patsubst %.tex,%.aux,$(wildcard *.tex))


.PHONY: default run_latexmk run_pdflatex run_latex dvipdf dvips clean cleanpdf cleanps cleanall cleanpstopdf help

#-------------------------------------------------------------------------------
# Default target - make mydocument.pdf with latexmk.
default: run_latexmk
# Use pdflatex/biber instead to compile.
#default: run_pdflatex

# Remove -pdf option to run latex instead of pdflatex
run_latexmk:
	latexmk -pdf $(BASENAME)

# Standard pdflatex target
run_pdflatex: $(BASENAME).pdf
	@echo "Made $<"

# Specify the tex and bib file dependencies for running pdflatex
#%.pdf: %.tex  $(tex_files) $(graphics_pdf)
%.pdf: %.tex
	$(PDFLATEX) -file-line-error $<
	-$(BIBTEX)  $(basename $<)
	$(PDFLATEX) $<
	$(PDFLATEX) $<

#-------------------------------------------------------------------------------
run_latex: dvipdf

# Targets if you run latex instead of pdflatex
dvipdf: $(BASENAME).dvi
	$(DVIPDF) -sPAPERSIZE=a4 -dPDFSETTINGS=/prepress $<
	@echo "Made $(basename $<).pdf"

dvips:  $(BASENAME).dvi
	$(DVIPS) $<
	@echo "Made $(basename $<).ps"

# Specify dependencies for running latex
%.dvi:  %.tex *.tex *.bib $(BASENAME)-defs.sty
	$(LATEX)    $<
	-$(BIBTEX)  $(basename $<)
	$(LATEX)    $<
	$(LATEX)    $<

%.bbl:  %.tex *.bib
	$(LATEX) $<
	$(BIBTEX) $<

#-------------------------------------------------------------------------------
help:
	@echo "To compile the paper (using pdflatex) give the command"
	@echo "make"
	@echo ""
	@echo "To compile the paper (using latex) give the command"
	@echo "make run_latex"
	@echo ""
	@echo "make clean    to clean auxiliary files (not output PDF)"
	@echo "make cleanpdf to clean output PDF files"
	@echo "make cleanps  to clean output PS files"
	@echo "make cleanall to clean all files"
	@echo "make cleanepstopdf to clean PDF files automatically made from EPS"
	@echo ""

clean:
	-rm -f *.dvi *.toc *.aux *.log *.out \
	*.bbl *.blg *.brf *.bcf *-blx.bib *.run.xml \
	*.cb *.ind *.idx *.ilg *.inx \
	*.synctex.gz *~ *.fls *.fdb_latexmk .*.lb spellTmp \
	$(TEXDIR)/*~ $(TEXDIR)/*.aux

cleanpdf:
	-rm -f $(BASENAME).pdf

cleanps:
	-rm -f $(BASENAME).ps

cleanall: clean cleanpdf cleanps

# Clean the PDF files created automatically from EPS files
cleanepstopdf: $(EPSTOPDFFILES)
	@echo "Removing PDF files made automatically from EPS files"
	-rm $^

